Novel Tetrahedral Human Phantoms for Space Radiation Dose Assessment

Space radiation remains one of the primary hazards to spaceflight crews. The unique nature of the intravehicular radiation spectrum makes prediction of biological outcomes difficult, with computational simulation-based efforts stymied by lack of computational resources or accurate modeling capabilities. Recent advancements in both Monte Carlo simulations and computational human phantom developments have allowed for complex radiation simulations and dosimetric calculations to be performed for numerous applications. In this work, advanced tetrahedral-type human phantoms were exposed to a simulated spectrum of particles equivalent to a single days exposure in the International Space Station in Low Earth Orbit. 3D Monte Carlo techniques were used to produce and simulate the radiation spectra. Organ absorbed dose, average energy deposition, and the whole-body integral dose was determined for a male and female phantom. Results were then extrapolated for two long-term scenarios: a 6-9 month mission on the International Space Station and a 3-year mission to Mars. The whole-body integral dose for the male and female models were found to be 0.2985 +- 0.0002 mGy/day 0.3050 +- 0.0002 mGy/day, respectively, which is within 10% of recorded dose values from the International Space Station. This work presents a novel approach to assess absorbed dose from space-like radiation fields using high-fidelity computational phantoms, highlighting the utility of complex models for space radiation research.

==> bibliography.tex <==

\addcontentsline{toc}{chapter}{REFERENCES}

\renewcommand{\bibname}{{\normalsize\rm REFERENCES}}

\bibliographystyle{unsrt}
% \bibliography{references}
